Bootstrap3D: Improving Multi-view Diffusion Model with Synthetic Data

Recent years have witnessed remarkable progress in multi-view diffusion models for 3D content creation. However, there remains a significant gap in image quality and prompt-following ability compared to 2D diffusion models. A critical bottleneck is the scarcity of high-quality 3D objects with detailed captions. To address this challenge, we propose Bootstrap3D, a novel framework that automatically generates an arbitrary quantity of multi-view images to assist in training multi-view diffusion models. Specifically, we introduce a data generation pipeline that employs (1) 2D and video diffusion models to generate multi-view images based on constructed text prompts, and (2) our fine-tuned 3D-aware MV-LLaVA for filtering high-quality data and rewriting inaccurate captions. Leveraging this pipeline, we have generated 1 million high-quality synthetic multi-view images with dense descriptive captions to address the shortage of high-quality 3D data. Furthermore, we present a Training Timestep Reschedule (TTR) strategy that leverages the denoising process to learn multi-view consistency while maintaining the original 2D diffusion prior. Extensive experiments demonstrate that Bootstrap3D can generate high-quality multi-view images with superior aesthetic quality, image-text alignment, and maintained view consistency.

==> subtex/statements.tex <==
\section{Ethics Statement}
Our training code is modified based on public available repository \url{https://github.com/PixArt-alpha/PixArt-alpha}. Part of training data are synthesized by our proposed data generation pipeline. For other part of original Objaverse~\cite{deitke2023objaverse} data, we only use Cap3D~\cite{luo2024scalable} filtered assets (Objects with CC BY-NC-SA and CC BY-NC licenses are removed, while we retain those with CC-BY 4.0, CC BY-SA, and CC0 licenses) and with face recognizable objects filtered through MSFW classifier and face detector. The ethical filtering in Cap3D make our work using only data without ethics problem. For our synthetic new data, We will launch both the generated captions for Objaverse~\cite{deitke2023objaverse} and high-quality synthetic data, model checkpoints and codes with CC-BY 4.0 license for the research community.

\section{Reproducibility Statement}
Main experimental setting/details (training data, hyperparameters, optimizer, evaluation settings, etc) are clearly presents in Sec.~\ref{sec:training_setting}. For main results, we detail the full test settings in Sec.~\ref{sec:test_setting}. For GPT-4V~\cite{2023GPT4VisionSC} based preference study, we provide detailed test prompts and test settings in Sup.~\ref{sup:gpt_evaluation}. Readers can easily follow the same settings and reproduce all of our experiment results. We provide code for generating synthetic data. Both codes for training the model and testing are also available in supplementary material. The full data and model checkpoints are too large to provide public link without violation of double-blinding. We will release full data and model checkpoints after review.
